Balancing Egoism and Altruism on the Interference Channel: The MIMO case

This paper considers the so-called MIMO interference channel. This situation has relevance in applications such as multi-cell coordination in cellular networks as well as spectrum sharing in cognitive radio networks among others. We address the design of precoding (i.e. beamforming) vectors at each sender with the aim of striking a compromise between beamforming gain at the intended receiver (Egoism) and the mitigation of interference created towards other receivers (Altruism). Combining egoistic and altruistic beamforming has been shown previously to be instrumental to optimizing the rates in a MISO interference channel (i.e. where receivers have no interference canceling capability) . Here we explore these game-theoretic concepts in the more general context of MIMO channels and using the framework of Bayesian games, allowing us to derive (semi-)distributed precoding techniques. We draw parallels with existing work on the MIMO interference channel, including rate-optimizing and interference-alignement precoding techniques, showing how such techniques may be improved and re-interpretated through a common prism based on balancing egoistic and altruistic beamforming.

==> chapter_IC.tex <==
\subsection{DBA Achieving Pareto Boundary}\label{subsection:pb}
In the special case of 2-link MISO system, the transmit beamformers $\mathbf{w}_i(t)$ for each iteration $t$ is a linear combination of the egoistic solution: MRC and altruistic solution : zero-forcing solution. Such transmit beamformers have the following equivalent representation, (for details, please refer to \cite{Randa2008})
\begin{equation}
 \mathbf{w}_1=\sqrt{\zeta_1}\frac{\Pi_{12}\mathbf{h}_{11}^H}{|\Pi_{12}\mathbf{h}_{11}^H|} +\sqrt(1-\zeta)\frac{\Pi_{12}^\perp \mathbf{h}_{11}^H}{|\Pi_{12}^\perp \mathbf{h}_{11}^H|}
\end{equation}
and similarly for $\mathbf{w}_2$. $\Pi_{12}$ is a projection matrix on $\mathbf{h}_{12}$ which is a row vector of channel gains from Tx $1$ to Rx $2$. Also, $\zeta_1 \in (0, \frac{a_1}{a_1+b_1})$ where $a_1= |\Pi_{12} \mathbf{h}_{11}^H|^2$, $b_1= |\Pi_{12}^\perp \mathbf{h}_{11}^H|^2$.

Since $ |\mathbf{h}_{11}\mathbf{w}_1|^2 = \left( \sqrt{a_1 \zeta_1} + \sqrt{b_1(1-\zeta_1)}\right)^2$ and
$|\mathbf{h}_{12} \mathbf{w}_1|^2 = \zeta_1 |\mathbf{h}_{12}|^2$, 
the SINR of Rx 1 is $\gamma_1 = \rho \frac{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}{1+\zeta_2 c_2} $ where $c_1= \rho |\mathbf{h}_{12}|^2$ and similarly for Rx 2.
%\gamma_2 &= \rho \frac{\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)^2}{1+\zeta_1 c_1}

Differtiate $\gamma_1$ with respect to $\zeta_1, \zeta_2$, we have
$\frac{d\gamma_1}{d\zeta_1} = \rho \frac{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)}{1+\zeta_2 c_2} $ and
$\frac{d\gamma_1}{d\zeta_2} = -\rho \frac{c_2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}{\left(1+\zeta_2 c_2\right)^2}$.Similar equations hold for $\gamma_2$.

If a point lies on the Pareto boundary, no increase in $\gamma_1$ can be accompanied by an increase in $\gamma_2$.
Note that the gradient of $\gamma_1$ is  $\gamma_1' = \gamma_1 + \delta_1 \frac{d\gamma_1}{d\zeta_1} + \delta_2 \frac{d\gamma_1}{d\zeta_2}$ and similarly for $\gamma_2$.
Thus, a point is on the Pareto bounday if the following equations hold at the same time:
$\delta_1 \frac{d\gamma_1}{d\zeta_1} + \delta_2 \frac{d\gamma_1}{d\zeta_2} > 0$ and
$\delta_1 \frac{d\gamma_2}{d\zeta_1} + \delta_2 \frac{d\gamma_2}{d\zeta_2} < 0$.

After some manipulation, they correspond to 
\begin{eqnarray}
& &\delta_1 \left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right) - \delta_2 \frac{c_2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}{\left(1+\zeta_2 c_2\right)} > 0\\
& & \delta_2\left(\frac{\sqrt{a_2}}{\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{\sqrt{1-\zeta_2}}\right) - \delta_1 \frac{c_1\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)}{\left(1+\zeta_1 c_1\right)} < 0 .
\end{eqnarray}
The inequalities are satisfied when 
%\begin{equation}
%\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)
%\left(\frac{\sqrt{a_2}}{\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{\sqrt{1-\zeta_2}}\right)= \frac{c_1\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)}{\left(1+\zeta_1 c_1\right)}
%\frac{c_2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}{\left(1+\zeta_2 c_2\right)}
%\end{equation}
%We can manipulate it into
\begin{equation}
\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)
\frac{\left(1+\zeta_1 c_1\right)}{c_1\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}
=\frac{\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)c_2}{\left(\frac{\sqrt{a_2}}{\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{\sqrt{1-\zeta_2}}\right)\left(1+\zeta_2 c_2\right)}
\end{equation}
The L.H.S is equal to infinity when $\zeta_1=0$ and zero when $\zeta_1=\frac{a_1}{a_1+b_1}$ whereas the R.H.S equals to infinity when $\zeta_2 = \frac{a_2}{a_2+b_2}$ and zero when $\zeta_2=0$.Since both of them are continuous functions (not necessarily monotonous), there exist some $\zeta_1, \zeta_2$ such that L.H.S equals to R.H.S.


%Taking the derivative of the left-hand side wrt $\zeta_1$:
%\begin{align}
%&-\frac{1}{2}\left(\frac{\sqrt{a_1}}{\zeta_1\sqrt{\zeta_1}}+\frac{\sqrt{b_1}}{(1-\zeta_1)\sqrt{1-\zeta_1}}\right)
%\frac{\left(1+\zeta_1 c_1\right)}{c_1}
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}
%\nonumber \\
%&+\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}
%\nonumber \\
%&-\frac{1}{2}\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)^2
%\frac{\left(1+\zeta_1 c_1\right)}{c_1}
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\nonumber \\
%&= -\frac{\left(1+\zeta_1 c_1\right)}{2c_1}
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\left[\frac{2a_1}{\zeta_1}+\frac{2b_1}{1-\zeta_1}+\sqrt{a_1b_1} \left[
%\frac{\sqrt{\zeta_1}}{(1-\zeta_1)^{3/2}}+\frac{\sqrt{1-\zeta_1}}{\zeta_1^{3/2}}-\frac{2}{\sqrt{\zeta_1(1-\zeta_1)}}
%\right]\right]
%\nonumber \\
%&+\frac{
%a_1-b_1+\sqrt{a_1b_1}\frac{1-2\zeta_1}{\sqrt{\zeta_1(1-\zeta_1)}}
%}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\nonumber \\
%&= -\frac{\left(1+\zeta_1 c_1\right)}{2c_1}
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\left[\frac{2a_1}{\zeta_1}+\frac{2b_1}{1-\zeta_1}+
%\frac{\sqrt{a_1b_1}(1-2\zeta_1)^2}{\zeta_1^{3/2}(1-\zeta_1)^{3/2}}\right]\nonumber \\
%&+\frac{
%a_1-b_1+\sqrt{a_1b_1}\frac{1-2\zeta_1}{\sqrt{\zeta_1(1-\zeta_1)}}
%}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\nonumber \\
%&= -\frac{1}{2c_1}
%\frac{1}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2}
%\left[\frac{2a_1}{\zeta_1}+\frac{2b_1}{1-\zeta_1}+
%\frac{\sqrt{a_1b_1}(1-2\zeta_1)^2}{\zeta_1^{3/2}(1-\zeta_1)^{3/2}}\right]\nonumber \\
%&+
%\frac{\sqrt{b_1}}{\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)^2(1-\zeta_1)}
%\left[-\sqrt{b_1}+\frac{1}{2}\sqrt{a_1}\frac{1-2\zeta_1}{\sqrt{\zeta_1(1-\zeta_1)}}
%\right]\nonumber \\
%\end{align}


%Performing implicit differentiation:
%\begin{align}
%&\left(-\frac{\sqrt{a_1}}{2\zeta_1\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{2(1-\zeta_1)\sqrt{1-\zeta_1}}\right)
%\left(\frac{\sqrt{a_2}}{\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{\sqrt{1-\zeta_2}}\right)
%\nonumber \\
%&+\frac{c_1^2\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)}{\left(1+\zeta_1 c_1\right)^2}
%\frac{c_2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}{\left(1+\zeta_2 c_2\right)} \nonumber \\
%&-\frac{c_1\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)}{\left(1+\zeta_1 c_1\right)}
%\frac{c_2\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)} \nonumber \\
%&=-\frac{d\zeta_2}{d\zeta_1}\left(\frac{\sqrt{a_1}}{\sqrt{\zeta_1}}-\frac{\sqrt{b_1}}{\sqrt{1-\zeta_1}}\right)
%\left(-\frac{\sqrt{a_2}}{2\zeta_2\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{2(1-\zeta_2)\sqrt{1-\zeta_2}}\right)
%\nonumber \\
%&-\frac{d\zeta_2}{d\zeta_1}\frac{c_1\left(\sqrt{a_2 \zeta_2}+\sqrt{b_2 (1-\zeta_2)}\right)}{\left(1+\zeta_1 c_1\right)}
%\frac{c_2^2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}{\left(1+\zeta_2 c_2\right)^2} \nonumber \\
%&+\frac{d\zeta_2}{d\zeta_1}\frac{c_1\left(\frac{\sqrt{a_2}}{\sqrt{\zeta_2}}-\frac{\sqrt{b_2}}{\sqrt{1-\zeta_2}}\right)}{\left(1+\zeta_1 c_1\right)}
%\frac{c_2\left(\sqrt{a_1 \zeta_1}+\sqrt{b_1 (1-\zeta_1)}\right)}{\left(1+\zeta_2 c_2\right)} \nonumber \\
%\end{align}
